Inflating Topic Relevance with Ideology: A Case Study of Political Ideology Bias in Social Topic Detection Models

We investigate the impact of political ideology biases in training data. Through a set of comparison studies, we examine the propagation of biases in several widely-used NLP models and its effect on the overall retrieval accuracy. Our work highlights the susceptibility of large, complex models to propagating the biases from human-selected input, which may lead to a deterioration of retrieval accuracy, and the importance of controlling for these biases. Finally, as a way to mitigate the bias, we propose to learn a text representation that is invariant to political ideology while still judging topic relevance.

==> tables/bq_table_result_ration_new.tex <==
\begin{table}
\centering
\begin{tabular}{cc|c||c|c}
\cline{2-5}
&\multicolumn{2}{c||}{\textbf{Immigration}}&\multicolumn{2}{c}{\textbf{Gun control}}\\\cline{2-5}
&\textit{Blue}-leaning Train&\textit{Red}-leaning Train & \textit{Blue}-leaning Train & \textit{Red}-leaning Train\\
\hline

GloVe&
1.99&
1.11&
2.27&
0.92\\
GloVe+ADV&
\textbf{1.72}&
\textbf{1.07}&
\textbf{2.17}&
\textbf{1.01}\\\hline
ELMo&
1.83&
1.15&
2.31&
0.98\\
ELMo+ADV&
\textbf{1.68}&
\textbf{0.89}&
\textbf{1.42}&
\textbf{1.01}\\\hline
BERT&
1.85&
1.15&
2.56&
1.05\\
BERT+ADV&
\textbf{1.77}&
\textbf{1.13}&
\textbf{2.02}&
\textbf{1.00}\\
\hline
\end{tabular}

\caption{\emph{Blue}-versus-\emph{Red} \textit{Odds Ratio} of original and our proposed models trained on \textit{Blue}-leaning or \textit{Red}-leaning training sets. Our proposed model is bolded if it outperforms its base model (the closer to 1, the better).}
\label{tab:ratio_new}
\end{table}
